CollaChain: A BFT Collaborative Middleware for Decentralized Applications

The sharing economy is centralizing services, leading to misuses of the Internet. We can list growing damages of data hacks, global outages and even the use of data to manipulate their owners. Unfortunately, there is no decentralized web where users can interact peer-to-peer in a secure way. Blockchains incentivize participants to individually validate every transaction and impose their block to the network. As a result, the validation of smart contract requests is computationally intensive while the agreement on a unique state does not make full use of the network. In this paper, we propose Collachain, a new byzantine fault tolerant blockchain compatible with the largest ecosystem of DApps that leverages collaboration. First, the pariticipants executing smart contracts collaborate to validate the transactions, hence halving the number of validations required by modern blockchains (e.g., Ethereum, Libra). Second, the participants in the consensus collaborate to combine their block proposal into a superblock, hence improving throughput as the system grows to hundreds of nodes. In addition, Collachain offers the possibility to its users to interact securely with each other without downloading the blockchain, hence allowing interactions via mobile devices. Collachain is effective at outperforming the Concord and Quorum blockchains and its throughput peaks at 4500 TPS under a Twitter DApp (Decentralized Application) workload. Finally, we demonstrate Collachain's scalability by deploying it on 200 nodes located in 10 countries over 5 continents.

==> alg/Algo0.tex <==
\begin{algorithm}[h!]
%	\caption{Client\label{alg:sevm}}
	{\footnotesize
	\begin{algorithmic}[1]
	
		\Part{$\lit{balance}(\ms{account})$}\Comment{client request to retrieve the correct balance of an account}
			\State Let $P$ be a set of $2t+1$ SEVM nodes \Comment{to $2t+1$ SEVM nodes}
			\ForAll{$p_j \in P$}   		
				  $\lit{send}(\lit{read}, \ms{account})$ to $p_j$ \Comment{multicast read message} \label{line:multicast}
			\EndFor
			\WUntil{received same balance response $b$ from $t+1$ distinct nodes} \label{line:enough-responses} \EndWUntil 
%			\If{$\exists b_1, b_2 \in B_1 ~|~ b_1 \neq b_2$} \label{line:detect-difference} \Comment{detect different responses}
%				\WUntil{received balance responses $B_2$ from $2t+1$ distinct nodes}\EndWUntil
%				\State $\ms{result} \gets b ~|~ b$ is the majority value among the responses in $B_2$  \label{line:different-copy}
%			\Else{}
%				 $\ms{result} \gets b ~|~ b \in B_1$ \label{line:same-copy} \Comment{pick any of the identical copies}
%			\EndIf
			\Return $\ms{b}$ \Comment{return balance} 
			\EndReturn
			
		\EndPart
		
		\Statex
	
		\Part{$\lit{send}(\ms{tx})$}\Comment{client request to send tx (e.g., smart contract invocation/upload)} \label{line:send-start}
			\State Let $p_j$ be one of the SEVM nodes in my neighborhood  \Comment{to 1 neighbor}	
			\State $\lit{send}(\lit{write}, \ms{tx})$ to $p_j$ \Comment{best effort send of a write operation} \label{line:send-end}
		\EndPart
		
		\algstore{alg:blockchain0}
	
	\end{algorithmic}%
}%
\end{algorithm}%

==> alg/Algo1.tex <==
\begin{algorithm}[h!]
%	\caption{SEVM\label{alg:sevm}}
	{\footnotesize
	\begin{algorithmic}[1]
	
		\algrestore{alg:blockchain0}

		\Part{$\lit{receive}(tx)$}\Comment{SEVM upon receiving a transaction}
		\If{$\lit{is-evalid}$} \Comment{if tx is eagerly validated}
		  	\State $\ms{mempool} \gets \ms{mempool} \cup \ms{tx}$  \Comment{add it to mempool}
		\EndIf

		\WUntil{|$\ms{mempool}$| = $\lit{threshold}$ or ${timer}$ expired}\Comment{wait sufficiently}\EndWUntil  %until threshold number of txs are received or timeout has reached}
		
		\ForAll{$\ms{tx}$ in $\lit{mempool}$} 
		$\ms{props} \gets \ms{props} \cup \{\ms{tx}\}$ \Comment{create proposal} %with valid txs}
		\EndFor

	
		\State $\ms{props} \gets \ms{props} \cup \{{timestamp}\}$ \Comment{add timestamp to proposal}

		\State $\ms{superblock} \gets \lit{propose}(\ms{props})$ \Comment{propose to consensus, return superblock}
        
       		\State $\lit{exec}(\ms{superblock})$ \Comment{execute superblock}
		
		\EndPart
		
		\algstore{alg:blockchain1}
	
	\end{algorithmic}%
}%
\end{algorithm}%

==> alg/Algo2.tex <==
\begin{algorithm}[h!]
%	\caption{Consensus\label{alg:consensus}}
	{\footnotesize
	\begin{algorithmic}[1]
	
	
	\algrestore{alg:blockchain2}

		\Part{$\lit{propose}(\ms{props})$}\Comment{starting the consensus algorithm}
		\State $\lit{reliable-broadcast}(\ms{props}) \to \ms{props[k]}$ \Comment{reliably deliver in $\ms{props}$ array}
		\While{$|\{k : \ms{bitmask}[k]=1\}|< n-t$ or ${timer}$ did not expire}
				\State {\bf for all}~{$k$ such that $\ms{props}[k]$ has been delivered}
				\State \T$\ms{bitmask}[k] \gets \lit{bin-propose}_k(1)$\Comment{propose 1 to binary consensus~\cite{CGLR18}}
        \EndWhile
        \State {\bf for all}~{$k$ such that $\ms{props}[k]$ has not been delivered}
        \State \T $\ms{bitmask}[k] \gets \lit{bin-propose}_k(0)$ \Comment{propose 0 to $k^{\ms{th}}$ binary consensus}
        \WUntil{$\ms{bitmask}$ is full and $\forall \ell,\ms{bitmask}[\ell] = 1 : \ms{props}[\ell] \neq \emptyset$}\EndWUntil  
        \Part{$\forall \ell s.t. \ms{props}[\ell] \neq \emptyset$}
        $\ms{superblock} \cup \ms{props[\ell]}$ \Comment{Add proposal to superblock}
        \EndPart
		\EndPart
		
	
	\end{algorithmic}%
	}%
\end{algorithm}%

==> alg/Algo3.tex <==
\begin{algorithm}[h!]
%	\caption{SEVM execution\label{alg:sevmexecution}}
	{\footnotesize
	\begin{algorithmic}[1]
	
	\algrestore{alg:blockchain1}

		\Part{$\lit{exec}(\ms{superblock})$}\Comment{parse superblock to the SEVM}
	    \ForEach{$\ms{props[k]}$ in $\ms{superblock}$}
	     \ForAll{$tx$ in $\ms{props[k]}$}
	     		\If{$\lit{is-lvalid}(tx)$} \Comment{if lazy validated}
				%\State $\tup{\ms{S_{next_{k}}}, \ms{receipt}} \gets \lit{run}(\ms{tx}, \ms{S})$ \Comment{exec, return state  receipt}
	     			\State$\ms{receipts_{k}} \gets \ms{receipts_{k}} \cup \{receipt\}$\Comment{collect all receipts}
	     			\State$\ms{val_{k}} \gets \ms{val_{k}} \cup \{tx\}$\Comment{collect executed txs from $\ms{props[k]}$ to $\ms{val_{k}}$}
	     		\EndIf
	     \EndFor
	     \State$\ms{TX}_{k}$ $\gets$ $\lit{update-tx-trie(val_{k})}$\Comment{update transaction trie}
	     \State$R_{k}$ $\gets$ $\lit{update-receipt-trie(receipts_{k})}$\Comment{update transaction receipt trie}
	     \State$B_{l}$ $\gets \langle h(\lit{header}(B_{l-1})), h(\ms{S_{next_{k}}}), h(\ms{TX}_{k}), h(R_{k}), \ms{GU}_{k}, \ms{GL},$ 
	     \State \T\T\T$\ms{nonce}, \ms{timestamp}_{k}, \ms{val}_{k}\rangle $ \Comment{create block}
	     
	     \State $\ms{chain} \gets \ms{chain} \cup B_{k}$
	    \EndFor
		\EndPart
		
		
	\algstore{alg:blockchain2}
	
	\end{algorithmic}%
}%
\end{algorithm}%

==> alg/STV.tex <==
\begin{algorithm}[h!]
	\caption{Single Transferable Vote - Part 1\label{alg:stv}}
	{\footnotesize
	\begin{algorithmic}[1]
        \Part{Declarations}
        \State$Ballot_{i} = [X, Y, Z, ..]$ is the $i^{th}$ ballot $\mid$ $X,Y,Z$ are candidates
        \State$Ballot_{i}[k]$ is the $(k+1)^{th}$ preference of $Ballot_{k}$
        \State $size$ is the number of candidate preferences in a ballot
        \State $quota = (n-t)/(seats + 1)$ $\mid$ $n$ is the total number of consensus nodes of which $t$ are byzantine and $seats$ are the number of candidates that require to be elected
        \State $\ms{ballot-count}, select = 0$
        \State $threshold = n-t$
        \State $S=\{X,Y, Z, . . .\} \mid S$ is the set of candidates
        \EndPart
        \State
        \Part{$\lit{createCommittee}(Ballot_{i})$}
        \State$\ms{ballot-count} = \ms{ballot-count} + 1$
        \If{$\ms{ballot-count} = \ms{threshold}$}   \Comment{if ballots received equals threshold}
        %\ForAll{$i=0; i < \ms{ballot-count}; pref_{i}=0$}  \Comment{start from first preference}
        \ForAll{$i=0; i < \ms{ballot-count};i++$} 
        \State $\ms{pref}_{i}=0$
        \If{$Ballot_{i}$[$pref_{i}$]=$c$ $\mid c$ is in $\lit{S}$}
        votes[$c$]=votes[$c$] + 1\Comment{calculate votes for candidate $c$ for first preference}
        \EndIf
        \EndFor
        \State$round=0$
        \While{$|selected| < seats$}\Comment{do until the elected nodes equal the seats available}
        	\State$\lit{STV()}$
        	\State$round = round +1$
        	\If{$|S|-|eliminated| = seats$}\Comment{break the loop since if more are eliminated seats cannot be filled}
        		\State break
        	\EndIf
        \EndWhile
        
        \ForAll{$k=0; k< \ms{size};k++$}
        \ForAll{$i=0; i < \ms{ballot-count};i++$}
        \If{$|selected| < seats$ and
               $Ballot_{i}[k]=c \mid c$ is in $\lit{S}$, not in $\lit{selected}$ and not in $\lit{eliminated}$}
           \State $\lit{selected} \gets \lit{selected} \cup \{c\}$
        \EndIf
        \EndFor
        \EndFor
        
        \EndIf
        
        \EndPart
        
        \algstore{stv}
        
	\end{algorithmic}%
}%
\end{algorithm}%
\begin{algorithm}[h!]
	\caption{Single Transferable Vote - Part 2\label{alg:stv1}}
	{\footnotesize
	\begin{algorithmic}[1]
	
        \algrestore{stv}
        
        \Part{$\lit{STV}()$}
        \If{$\exists c \mid \lit{votes[c]} \geq quota$}\Comment{if the quota is equalled or exceeded}
         \State $\lit{selected} \gets \lit{selected} \cup \{c\}$\Comment{elect candidate}
        \If{$\lit{votes[c]} > quota$}
        	\State $\ms{excess-candidates}\gets \ms{excess-candidates} \cup \{c\}$\Comment{save candidates that exceed quota in $\ms{excess-candidates}$}
            \State$\ms{excess-vote_{c}} \gets \lit{votes[c]} - quota$\Comment{excess vote from candidate $c \mid c \exists$ in $\lit{S}$}
        \EndIf
        
        \State $\forall i$ 
        \If{$Ballot_{i}[pref_{i}]=c$ and $c \in \ms{excess-candidates}$}\Comment{If the current preference of the ballot is one of the excess candidates}
        \State$\ms{count{c}} \gets \ms{count_{c}} + 1$\Comment{The number of candidates $c$}
        $\ms{pref-next}_{i} \gets \ms{pref}_{i} + 1$
        \While{$Ballot_{i}[\ms{pref-next}_{i}] \not\in (selected \cup eliminated$)}\Comment{Increment the preference pointer until a non eliminated non selected candidate is found}
        \State $\ms{pref-next}_{i} \gets \ms{pref-next}_{i} + 1$
        \EndWhile
        %\State $\ms{pref-next}_{i} \gets \ms{pref}_{i} + 1$ %\Until{$Ballot_{i}[\ms{pref-next}_{i}] \not\in selected \not\in eliminated$}
        
        \If{$Ballot_{i}[pref_{i}]=c$ and $c \in \ms{excess-candidates}$ and $Ballot_{i}[\ms{pref-next}_{i}] \not\in  \lit{selected} \cup \lit{eliminated}$}
        \State $\ms{pref_{i}} =\ms{pref-next}_{i}$\Comment{move the preference pointer}
        \State $z \gets Ballot_{i}[\ms{pref}_{i}]$
        \State $candidates-next \gets candidates-next \cup (c,z)$\Comment{A tuple of the current candidate and the next candidate} 
        \State$\ms{count_{z}} \gets \ms{count_{z}} + 1$\Comment{The number of candidates $z$}
        \EndIf
        \EndIf
        
        \ForAll{unique $(c,z) \in \ms{candidates-next}$}
        \State$\lit{vote(z)} \gets \lit{vote(z)} + \ms{excess-vote_{c}} \cdot (count_{z}/\ms{count{c}})$\Comment{transfer excess votes to the next valid preference of the ballots}
        \EndFor
        
        \EndIf
         %\EndIf
        
        \If{$\forall c : votes[c] < quota$}\Comment{There are no candidates reaching the quota in the round}
        \State $\ms{eliminated} \gets \ms{eliminated} \cup t \mid t = \lit{min_{\forall c}(votes[c])}$\Comment{eliminate the candidate with the least votes}
        \State $\ms{transfer-vote} \gets \lit{votes[t]}$
        \State $\lit{votes[t] \gets 0}$\Comment{Assign votes of least candidate to 0}
         \ForAll{$k=0; k<size;k++$}
         	\ForAll{$i=0; i < \ms{ballot-count};i++$}
         		\If{$Ballot_{i}[k]=t$}
         			$elimpointer \gets elimpointer\cup (i,k)$\Comment{Store tuples of ballot number and preference index that references least voted candidate}
         		\EndIf
         	\EndFor
         \EndFor
         
         \If{$\exists (v,k) \in elimpointer \mid Ballot_{v}[k]=m$ and $m \in \ms{eliminated}$}\Comment{If the preference $k$ of the ballot $v$ is eliminated}
         \State $\ms{pref-next}_{v}=k+1$
         \State $\ms{count{m}} \gets \ms{count_{m}} + 1$\Comment{The number of candidates $m$}
         \While{$Ballot_{v}[pref-next_{v}] \not\in (selected \cup eliminated)$}\Comment{Increment the preference pointer until a non eliminated non selected candidate is found}
         \State $\ms{pref-next}_{v} \gets \ms{pref-next}_{v} + 1$
         \EndWhile
         %\Until{$Ballot_{v}[pref-next_{v}] \not\in selected \not\in eliminated$}
         
         \If{$Ballot_{v}[\ms{pref-next}_{v}] \not\in  \lit{selected} \cup \lit{eliminated}$}
         \State $pref_{v}\gets \ms{pref-next}_{v}$\Comment{move the preference pointer}
         \State $z \gets Ballot_{i}[\ms{pref}_{v}]$
         \State $candidates-next \gets candidates-next \cup (m,z)$\Comment{A tuple of the least voted candidate and the next candidate in ballot} 
         \State$\ms{count_{z}} \gets \ms{count_{z}} + 1$\Comment{the number of candidates $z$}
         \EndIf
         \EndIf
        
        \ForAll{unique $(m,z) \in candidates-next$}
        \State$\lit{vote(z)} \gets \lit{vote(z)} + \ms{transfer-vote} x (\ms{count_{z}}/\ms{count_{m}})$\Comment{transfer votes from the least voted candidate to next preference in their ballots.}
        \EndFor
        
        \EndIf
        \EndPart
	
	\end{algorithmic}%
}%
\end{algorithm}%
